The Hidden Costs of Automation: An Empirical Study on GitHub Actions Workflow Maintenance

GitHub Actions (GA) is an orchestration platform that streamlines the automatic execution of software engineering tasks such as building, testing, and deployment. Although GA workflows are the primary means for automation, according to our experience and observations, human intervention is necessary to correct defects, update dependencies, or refactor existing workflow files. In fact, previous research has shown that software artifacts similar to workflows, such as build files and bots, can introduce additional maintenance tasks in software projects. This suggests that workflow files, which are also used to automate repetitive tasks in professional software production, may generate extra workload for developers. However, the nature of such effort has not been well studied. This paper presents a large-scale empirical investigation towards characterizing the maintenance of GA workflows by studying the evolution of workflow files in almost 200 mature GitHub projects across ten programming languages. Our findings largely confirm the results of previous studies on the maintenance of similar artifacts, while also revealing GA-specific insights such as bug fixing and CI/CD improvement being among the major drivers of GA maintenance. A direct implication is that practitioners should be aware of proper resource planning and allocation for maintaining GA workflows, thus exposing the ``hidden costs of automation.'' Our findings also call for identifying and documenting best practices for such maintenance, and for enhanced tool features supporting dependency tracking and better error reporting of workflow specifications.

==> old_research-questions.tex <==
\section{Research Questions}

The \emph{goal} of this study is to characterize the effort needed to maintain GitHub Actions workflow files. The context consists of the change history of 183 projects hosted on GitHub using GA across 10 programming languages over a period of four years. Our \emph{purpose} is threefold: first, to measure the \emph{distribution and number of workflow files}, which refers to the size and frequency of changes between workflow files and other file categories, such as production and test code, second, to examine the \emph{workflow coupling}, which denotes the degree of interdependence between workflow files and other file categories, and third, to assess \emph{workflow ownership}\pv{*} by identifying the developers responsible for making these changes. Our methodology aligns with prior research on the maintenance of Build and Infrastructure as Code artifacts~\cite{mcintosh2011empirical,jiang2015co}.

Based on our study goal, we formulated the following Research Questions (RQs).

\textbf{RQ\textsubscript{1}: How many workflow files does a project have, and what is the NLOC?} 

We aim to quantify the presence of workflow files to assess their significance across multiple projects by considering two key metrics: Proportion and Number of Lines of Code (NLOC). Proportion is the ratio of workflow files to the total files in a project. NLOC is the number of lines within each of these workflow files.


\textbf{RQ\textsubscript{2}: What is the Churn rate of workflow files?} 

In addition to quantifying the presence of Workflow files, we seek to analyze the rate of change in these files, known as Churn, which can provide insights into the extent to which developers modify workflows. Previous research by Shin \etal, and Jiang and Adams~\cite{shin2010evaluating, jiang2015co} underscores that a high Churn rate may indicate the presence of flawed or potentially vulnerable files, requiring increased maintenance effort. Similarly, since workflow files are prone to errors and are challenging to debug~\cite{saroar2023developers}, they might exhibit a change rate that reflects the effort involved in correcting errors or debugging.


\textbf{RQ\textsubscript{3}: To what extent are workflow files coupled with other source code files?} 

Besides the presence and Churn of Workflow files, we also want to examine the degree of interdependence between workflow files and other file categories using logical coupling~\cite{gall1998detection}. 
Therefore, we refer to Workflow coupling as the degree of interdependence between workflow files and other file categories, such as production and test files. 
Previous studies indicate that artifacts similar to workflows, such as Build and Infrastructure as Code files, exhibit low coupling with source code files~\cite{jiang2015co,mcintosh2011empirical}. In this context, we aim to determine whether this is different for workflow files or holds true for them as well.

\textbf{RQ\textsubscript{4}: What are the reasons that contribute to the coupling between production, test, and workflow files?}

We aim to uncover the causes of coupling between workflow and other file categories. By knowing the reasons behind the coupling across multiple projects, we can assess whether it is an inherent aspect of the system architecture or if there is a common pattern of developers' behaviour.


\textbf{RQ\textsubscript{5}: How is workflow ownership distributed among developers?} 

In this RQ, we want to identify who maintains workflow files by examining the ownership distribution across multiple projects. Knowing this distribution can help us determine how many developers are involved in maintaining these artifacts.

==> old_tables.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table*}
\centering
\caption{Summary statistics for production, test, and workflow file proportions for both single and multi-project groups.}
\label{tab:rq1a}
\begin{tabularx}{\textwidth}{llYYYYYYY}
\toprule
 & & \multicolumn{3}{c}{Group Multi} & \multicolumn{3}{c}{Group Single} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
 & & Production & Test & Workflow & Production  & Test  & Workflow  \\
\midrule
\multirow{4}{*}{Statistics} 

 & 1st Quartile & 61.4544  & 3.5541 & 0.4317 & 74.3421 & 0.0000 & 0.3609 \\
 & Mean & 74.5971 & 21.6535 & 3.7492 & 83.3144 & 13.6310 & 3.0545 \\
 & Median & 77.1768 & 20.0569  & 1.1118 & 92.1052  & 2.0366  & 0.8547 \\
 & 3rd Quartile & 93.3259 & 33.0069 & 2.8879 & 98.4884 & 18.5827  & 2.2773 \\
\bottomrule
\end{tabularx}
\end{table*}


\begin{table}
\centering
\caption{NLOC distribution of the three file categories.}
\label{tab:NLOC}
\begin{tabular}{lrrrrr}
\toprule
 & & Production & Test & Workflow \\
\midrule
\multirow{4}{*}{Group Multi} 
 %& Count & 5718 & 5718 & 5718 \\
 & 1st Quartile & 37.8750  & 49.0000  & 36.7500   \\
 & Mean & 103.2564 & 101.3682 & 60.9967 \\
 & Median & 61.0000  & 82.0000  & 46.5000 \\
 & 3rd Quartile & 112.6250  & 123.2500  & 67.5000 \\

\midrule
\multirow{4}{*}{Group Single} 
 %& Count & 680 & 680 & 680 \\
 & 1st Quartile & 49.2500  & 44.5000 & 36.0000   \\
 & Mean & 128.1851 & 113.3157 & 98.9259 \\
 & Median & 103.0000 & 126.0000 & 68.0000 \\
 & 3rd Quartile & 139.2500 & 164.0000  & 128.0000 \\

\bottomrule
\end{tabular}
\end{table}


\begin{table}[ht!]
\centering
\caption{The proportion of files on each of the three file categories.}
\label{tab:CHURN}
\begin{tabular}{lrrrrr}
\toprule
 & & Production & Test & Workflow \\
\midrule
\multirow{4}{*}{Group Multi} 
 %& Count & 5718 & 5718 & 5718 \\
 & 1st Quartile & 0.6111 & 0.0000 & 0.0000 \\
 & Mean & 0.7412 & 0.1890 & 0.0828 \\
 & Median & 0.8057 & 0.1176 & 0.0068 \\
 & 3rd Quartile & 0.9576 & 0.3199 & 0.0425 \\

\midrule
\multirow{4}{*}{Group Single} 
 %& Count & 680 & 680 & 680 \\
 & 1st Quartile & 0.8141 & 0.0000 & 0.0000 \\
 & Mean & 0.8453 & 0.1075 & 0.0695 \\
 & Median & 0.9655 & 0.0000 & 0.0000 \\
 & 3rd Quartile & 1.0000 & 0.1250 & 0.0067 \\

\bottomrule
\end{tabular}
\end{table}


\begin{table}[ht]
\centering
\begin{tabular}{lrr}
\toprule
\textbf{Category Combination} & \textbf{Chi-Square Value} & \textbf{p-value} \\ \midrule
Workflow \& Test & 4502.59 & 0.0 \\ 
Workflow \& Production & 78799.33 & 0.0 \\ 
Test \& Production & 58511.84 & 0.0 \\ 
\bottomrule
\end{tabular}
\caption{Results of Chi-Square Test.}
\label{tab:chi-square}
\end{table}

\begin{table}[t]
\centering
\caption{Association Rule metrics: Conf, Supp, and Lift~\cite{agrawal1993mining}.}
\begin{tabular}{>{\centering\arraybackslash}m{0.14\columnwidth}>{\centering\arraybackslash}m{0.14\columnwidth}>{\raggedright\arraybackslash}m{0.56\columnwidth}}
\toprule
\textbf{Metric} & \textbf{Formula} & \textbf{Description} \\
\midrule
 Conf(A$\Rightarrow$B) & $\frac{P(A \cap B)}{P(A)}$ & Determines how often changes in one file category occur along with changes in another \\
\midrule
Support(A,B) & $P(A \cap B)$ & Determines how frequently changes in two file categories occur together \\
\midrule
Lift(A$\Rightarrow$B) & $\frac{P(A \cap B)}{P(A)P(B)}$ & Determines the strength of the dependency between changes in two file categories \\
\bottomrule
\end{tabular}
\label{tab:ar_metrics}
\end{table}
